Scaling Distributed Ledgers and Privacy-Preserving Applications

This thesis proposes techniques aiming to make blockchain technologies and smart contract platforms practical by improving their scalability, latency, and privacy. This thesis starts by presenting the design and implementation of Chainspace, a distributed ledger that supports user defined smart contracts and execute user-supplied transactions on their objects. The correct execution of smart contract transactions is publicly verifiable. Chainspace is scalable by sharding state; it is secure against subsets of nodes trying to compromise its integrity or availability properties through Byzantine Fault Tolerance (BFT). This thesis also introduces a family of replay attacks against sharded distributed ledgers targeting cross-shard consensus protocols; they allow an attacker, with network access only, to double-spend resources with minimal efforts. We then build Byzcuit, a new cross-shard consensus protocol that is immune to those attacks and that is tailored to run at the heart of Chainspace. Next, we propose FastPay, a high-integrity settlement system for pre-funded payments that can be used as a financial side-infrastructure for Chainspace to support low-latency retail payments. This settlement system is based on Byzantine Consistent Broadcast as its core primitive, foregoing the expenses of full atomic commit channels (consensus). The resulting system has extremely low-latency for both confirmation and payment finality. Finally, this thesis proposes Coconut, a selective disclosure credential scheme supporting distributed threshold issuance, public and private attributes, re-randomization, and multiple unlinkable selective attribute revelations. It ensures authenticity and availability even when a subset of credential issuing authorities are malicious or offline, and natively integrates with Chainspace to enable a number of scalable privacy-preserving applications.

==> chapters/byzcuit/sections/background.tex <==
% ======
\section{Background and Related Work} \label{sec:byzcuit:background}
Replay attacks in general have seen extensive study in the security literature.
This work is the first that presents replay attacks on cross-shard consensus protocols.
Traditionally, the most stringent threat models assumed by consensus protocols involve Byzantine adversaries who are able to control or subvert consensus nodes and cause them to behave arbitrarily. 
Repurposing those protocols to cross-shard distributed ledgers (\eg, blockchains) opens up new attack avenues such as replay attacks as shown in Sections~\ref{sec:byzcuit:shard-led-consensus} and~\ref{sec:byzcuit:client-led-consensus}.

\subsection{Cross-Shard Consensus Protocols} \label{sec:byzcuit:cross-shard-consensus}
In sharded systems, some transactions may operate on objects handled by different shards, effectively requiring the relevant shards to additionally run a \emph{cross-shard consensus protocol} to enable agreement across the shards. Specifically, if any of the shards relevant to the transaction rejects it, all the other shards should likewise reject the transaction to ensure atomicity.

A typical choice for implementing cross-shard consensus is the two-phase atomic commit protocol~\cite{gray1978notes}. This protocol has two phases which are run by a \emph{coordinator}. In the first \emph{voting} phase, the nodes tentatively write changes locally, lock resources, and report their status to the coordinator. If the coordinator does not receive status message from a node (\eg, because the node crashed or the status message was lost), it assumes that the node's local write failed and sends a rollback message to all the nodes to ensure any local changes are reversed, and locks released. If the coordinator receives status messages from all the nodes, it initiates the second \emph{commit} phase and sends a commit message to all the nodes so they can permanently write the changes and unlock resources. In the context of sharded blockchains, the atomic commit protocol operates on shards (which make the local changes associated with the voting phase \via an intra-shard consensus protocol like PBFT), rather than individual nodes. A further consideration is who assumes the role of the coordinator; \emph{\clientled protocols} rely on the client to take the role of coordinator, and \emph{\shardled protocols} rely on entire shard.

There are currently two key approaches to cross-shard atomic commit protocols. The first approach involves \clientled protocols (such as \atomix~\cite{omniledger} and \rscoin~\cite{rscoin}), where the client acts as a coordinator. These protocols assume that clients are incentivized to proceed to the unlock phase. 
The second approach involves \shardled protocols (such as \sbac~\cite{chainspace} and Elastico~\cite{elastico}), where shards collectively assume the role of a coordinator.
All the concerned shards collaboratively run the protocol between them. This is achieved by making the entire shard act as a `resource manager' for the transactions it handles.
This chapter describes a family of replay attacks in the context of two representative systems: \sbac~\cite{chainspace}  
as an example of \shardled protocols (\Cref{sec:byzcuit:shard-led-consensus}); and \atomix as an example of \clientled protocols (\Cref{sec:byzcuit:client-led-consensus});
these attacks can compromise both system liveness and safety. 

\subsection{Mutex-Based Consensus Protocols}
Contrarily to \sbac and \atomix that achieve cross-shard consensus through a two-phase atomic commit protocol,
mutex-based schemes for cross-shard transactions, such as \rapidchain~\cite{rapidchain} and \ethereum's cross-shard `yanking' proposal~\cite{yanking}, adopt mutex-based schemes for transactions that involve objects managed by different shards.
The key idea is to require all objects that a transaction reads or writes  to be in the same shard (\ie, all locks for a transaction are local to the shard). Cross-shard transactions are enabled by transferring the concerned objects between shards, effectively giving shards a lock on those objects.  When shard 1 transfers an object to shard 2, shard 1 includes a transfer `receipt' in its blockchain. A client can then send to shard 2 a Merkle proof of this receipt being included in shard 1's blockchain, which makes the object active in shard 2.

Mutex-based schemes also need to consider replay attacks. Clients can claim the same receipt multiple times, unless shards store information about previously claimed receipts.  Na\"{\i}vely, shards have to store information about all previously claimed receipts permanently.
However, two intermediate options with trade-offs have been proposed~\cite{yanking}:
\begin{itemize}
    \item Shards only store information about receipts for $l$ blocks, and clients can only claim receipts within $l$ blocks; objects are permanently lost if not claimed in time (this introduces a synchrony assumption).
    \item Shards only store information about receipts for $l$ blocks, and include the root of a Merkle tree of claimed receipts in their blockchain every $l$ blocks. If a receipt is not claimed within $l$ blocks, the client must provide one Merkle proof every $l$ blocks that have passed to show that the receipt has not been previously claimed, in order to claim it. The longer the receipt was not claimed, the greater the number of proofs that are needed to claim a receipt. These proofs need to be also stored on-chain to allow other nodes to validate them.
\end{itemize}
\Cref{sec:byzcuit:byzcuit} presents a system, called \byzcuit, that forgoes the need for shards to store information about old state (such as inactive objects or old receipts) as shards only need to know the set of active objects they manage, and does not impose a trade-off between the amount of information about old state that needs to be stored and the cost of recovering old state that was held up in an incomplete cross-shard transaction (\ie, an unclaimed receipt).

        



==> chapters/chainspace/sections/abstract.tex <==
\chainspace is a decentralized infrastructure, known as a distributed ledger, that supports user defined smart contracts and executes user-supplied transactions on their objects. The correct execution of smart contract transactions is verifiable by all. The system is scalable, by sharding state and the execution of transactions, and using \sbac, a distributed commit protocol, to guarantee consistency. \chainspace is secure against subsets of nodes trying to compromise its integrity or availability properties through Byzantine Fault Tolerance (BFT), and extremely high-auditability, non-repudiation and `blockchain' techniques. Even when BFT fails, auditing mechanisms are in place to trace malicious participants. We present the design, rationale, and details of \chainspace; we argue through evaluating an implementation of the system about its scaling and other features; we illustrate a number of privacy-friendly smart contracts for smart metering, polling and banking and measure their performance. (\Cref{chainspace})

==> chapters/fastpay/sections/abstract.tex <==
\begin{abstract}
\fastpay allows a set of distributed authorities, some of which are Byzantine, to maintain a high-integrity and availability settlement system for pre-funded payments. It can be used to settle payments in a native unit of value (crypto-currency), or as a financial side-infrastructure to support retail payments in fiat currencies. \fastpay is based on Byzantine Consistent Broadcast as its core primitive, foregoing the expenses of full atomic commit channels (consensus). The resulting system has low-latency for both confirmation and payment finality. Remarkably, each authority can be sharded across many machines to allow unbounded horizontal scalability. Our experiments demonstrate intra-continental confirmation latency of less than 100ms, making \fastpay applicable to point of sale payments. In laboratory environments, we achieve a throughput of over 80,000 transactions per second with 20 authorities---surpassing the requirements of current retail card payment networks, while significantly increasing their robustness.
\end{abstract}

==> chapters/fastpay/sections/security_old.tex <==
% ======
% Security
% ======
\section{Security Analysis} \label{sec:fastpay:security}
Let $\sigma$ denote the current state of the \sysmain. We define $\funding^a(\sigma)$ as the sum of all the amounts transferred to a \fastpay address $a$ from the \sysmain:
\[
\funding^a(\sigma) \,=\, \sum_{\left\{\!\!\!\!\scriptsize\begin{array}{l} T \in \transactions(\sigma)\\ \recipient(T)=a \end{array}\right.} \amount(T)
\]
For simplicity, we write $\sum_C \amount(C)$ when we mean to sum over certified transfer orders: $\sum_{O \text { s.t. } \exists C. O = \val(C)} \amount(O)$.

The results presented in this section are proven in \Cref{sec:proofs}. We start with the main safety invariant of \fastpay.

\begin{theorem}[Solvency of \fastpay] \label{th:fastpay:theorem-s6} At any time, the sum of the amounts of all existing certified transfers from \fastpay to the \sysmain cannot exceed the funds collected by all transactions on the \sysmain smart contract:
\[
\sum_{\recipient(C) \in \sysmainaddresses} \!\!\amount(C)
\;\leq\; \sum_a \funding^a(\sigma)
\]
\end{theorem}

Next, we describe how receivers of valid transfer certificates can finalize transactions and make funds available on their own accounts (\sysmain and \fastpay).

\begin{proposition}[Redeemability of valid transfer certificates to \sysmain] \label{pr:fastpay:proposition-l1B}
A new valid \sysmain transfer certificate $C$ can always be redeemed by sending a new redeem transaction $T$ to the smart contract.
\end{proposition}

\begin{proposition}[Redeemability of valid transfer certificates to \fastpay] \label{pr:fastpay:proposition-l1A}
Any user can eventually have a valid \fastpay transfer certificate $C$ confirmed by any honest authority. \end{proposition}

Specifically, in \Cref{pr:fastpay:proposition-l1A}, the confirmation order for $C$ is guaranteed to succeed for every honest authority $\alpha$, provided that the user first recovers and transfers to $\alpha$ all the \emph{missing certificates required by $\alpha$}, defined as the sequence $C_k \ldots C_{n-1}$ such that $k = \nextsequencenumber^a(\alpha)$, $a = \sender(C)$, $n = \sequencenumber(C)$, $\sender(C_i) = a$ $(k\leq i \leq n-1)$. The fact that no other certificates need to be confirmed (\eg to credit the balance of $\sender(C)$ itself) is closely related to the possibility of (temporary) negative balances for authorities, and justified by the proof of safety in \Cref{sec:proofs}.

Note that having a \fastpay certificate confirmed by an authority $\alpha$ only affects $\alpha$'s recipient and the sender's balances (\ie \emph{redeems the certificate}) the first time it is confirmed.

Finally, we state that \fastpay funds credited on an account can always be spent.
%
We write $\received(a)$ for the set of \emph{incoming} transfer certificates $C$ such that $\recipient(C)=a$ and $C$ is known to the owner of the account\ $a$.

\begin{proposition}[Availability of transfer certificates] \label{pr:fastpay:proposition-l2}
Let $a$ be an account owned by a correct user, $n$ be the next available sequence number after the last signed transfer order (if any, otherwise $n=0$), and $O$ be a new transfer order signed by~$a$ with $\sequencenumber(O) = n$ and $\sender(O) = a$.

Assume that the owner of $a$ has secured enough funds for a new order $O$ based on their knowledge of the chain $\sigma$, the history of outgoing transfers, and the set $\received(a)$. That is, formally:
\[
\begin{array}{l}
\bigg( \amount(O) \; + \; \sum_{\left\{\!\!\!\!\scriptsize\begin{array}{l} \sender(C)=a\\ \sequencenumber(C) < n\end{array}\right.}\!\!\!\!\amount(C) \bigg) \\[0.4em]
\quad \leq \; \bigg( \funding^a(\sigma) \; + \; \sum_{C \in \received(a)} \amount(C) \bigg)
\end{array}
\]
Then, for any honest authority $\alpha$, the user will always eventually obtain a valid signature of $O$ from $\alpha$ after sending the following orders to $\alpha$:
\begin{enumerate}
\setlength\itemsep{0em}
\item A synchronization order from the \sysmain based on the known state $\sigma$;
\item A confirmation order for every $C \in \received(a)$, preceded by all the missing certificates required by $\alpha$ (if any) for the sender of $C$;
\item Then, the transfer order $O$.
\end{enumerate}
\end{proposition}

\para{Worst-case efficiency of \fastpay clients} To initiate a transfer (\Cref{proposition-l2}) or receive funds (\Cref{proposition-l1A}) from a sender account $a$, a \fastpay client must address a quorum of authorities. During the exchange, each authority $\alpha$ may require missing certificates $C_k \ldots C_{n-1}$, where $k = \nextsequencenumber^a(\alpha)$ is provided by $\alpha$. In an attempt to slow down the client, a Byzantine authority could return $k=0$ and/or fail to respond at some point. To address this, a client should query each authority $\alpha$ in parallel. After retrieving the sequence number~$k$, the required missing certificates should be downloaded sequentially, in reverse order, then forwarded to~$\alpha$. Given that \fastpay client operations succeed as soon as a quorum of authorities complete their exchanges, this strategy ensures client efficiency despite Byzantine authorities.
